Measuring the Exploitation of Weaknesses in the Wild

Identifying the software weaknesses exploited by attacks supports efforts to reduce developer introduction of vulnerabilities and to guide security code review efforts. A weakness is a bug or fault type that can be exploited through an operation that results in a security-relevant error. Ideally, the security community would measure the prevalence of the software weaknesses used in actual exploitation. This work advances that goal by introducing a simple metric that utilizes public data feeds to determine the probability of a weakness being exploited in the wild for any 30-day window. The metric is evaluated on a set of 130 weaknesses that were commonly found in vulnerabilities between April 2021 and March 2024. Our analysis reveals that 92 % of the weaknesses are not being constantly exploited.

==> ToDo.tex <==
Conference
    Identify conference
    Change paper to use conference template
    Initiate ERB review

Overall
    Go through all 130 CWEs and categorize by pattern
    Review CWE choices (and updated) for figures of pattern examples
    Identify target conference

Authors
    Get ORCID for Carlos

III Experiment Design
    Discuss CWE hierarchy
    Mention making mean calculations
    Describe the evaluation process / mashup better
    Differentiate on which patterns are determinable via an algorithm/equation/query
    Example query period when we are almost done and update figures/tables
    
IV Results
    Add figure on distribution of mean PECWE values
    Finalize CWEs for Table I, those we expect to include in discussion 
        (include examples w/ low PECWE and high CVE count and vice versa)

    IV A
        mention before that there is no data in EPSS for 2022-11-09.
        Add additional pattern types?
            Irena's new high-low, low-high patterns are different from
            Carlos' patterns. Need to distinguish!! Different columns in
            Table I!
        Update Table II
        Add additional figures for pattern examples (for new patterns)

    IV B
        update w/new Irena scatter plots, e.g. x<=800

V Discussion
    Write it!
    Discuss table II
    Discuss each example CWE in Table I and the related pattern figure
    Discuss scatterplots

Related Work?
    Add this section
    Write section/subsection on MITRE CWE Top 20
    Discuss NVD CWE statistics
    Do additional literature search

VI Conclusion
    Write it!
    


